Adapting Stereo Vision From Objects To 3D Lunar Surface Reconstruction with the StereoLunar Dataset

Accurate 3D reconstruction of lunar surfaces is essential for space exploration. However, existing stereo vision reconstruction methods struggle in this context due to the Moon's lack of texture, difficult lighting variations, and atypical orbital trajectories. State-of-the-art deep learning models, trained on human-scale datasets, have rarely been tested on planetary imagery and cannot be transferred directly to lunar conditions. To address this issue, we introduce LunarStereo, the first open dataset of photorealistic stereo image pairs of the Moon, simulated using ray tracing based on high-resolution topography and reflectance models. It covers diverse altitudes, lighting conditions, and viewing angles around the lunar South Pole, offering physically grounded supervision for 3D reconstruction tasks. Based on this dataset, we adapt the MASt3R model to the lunar domain through fine-tuning on LunarStereo. We validate our approach through extensive qualitative and quantitative experiments on both synthetic and real lunar data, evaluating 3D surface reconstruction and relative pose estimation. Extensive experiments on synthetic and real lunar data validate the approach, demonstrating significant improvements over zero-shot baselines and paving the way for robust cross-scale generalization in extraterrestrial environments.

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[per-mode=symbol]{siunitx}
\usepackage{xspace}
\usepackage{xcolor}

% \usepackage[capitalise,noabbrev]{cleveref}


\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\DeclareRobustCommand\nodot{\futurelet\@let@token\@nodot}
\def\@nodot{\ifx\@let@token.\else~\null\fi\xspace}

\newfont{\eaddfnt}{phvr8t at 12pt}
\def\email#1{{{\eaddfnt{\par #1}}}}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\pe{\textit{p.e}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\na{\emph{n.a}\onedot} \def\NA{\emph{N.A}\onedot}
\def\wrt{w.r.t\onedot} 
\def\dof{d.o.f\onedot}
\def\aka{a.k.a\onedot}
\def\phd{Ph.D\onedot}
\def\etal{\emph{et al}\onedot}

\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

\DeclareSIUnit\px{px}
\sisetup{
  output-decimal-marker = {.},   % or "," if you want decimal comma
  group-separator = {,},
  group-minimum-digits = 4
}

\newcommand{\commentaire}[1]{\textcolor{#1}}
\newcommand{\remarque}[2]{\commentaire{#1}{\textbf{[#2]}}}
\newcommand{\gm}{\commentaire{orange}} % Geraldine
\newcommand{\gmc}[1]{\remarque{orange}{(gm) #1}}
\newcommand{\gmrk}[1]{\gmc{\#1}}
\newcommand{\sg}{\commentaire{olive}} % Simone
\newcommand{\sgc}[1]{\remarque{olive}{#1}}
\newcommand{\cg}{\commentaire{magenta}} % Clementine
\newcommand{\cgc}[1]{\remarque{magenta}{(cg) #1}}
\newcommand{\cgrk}[1]{\cgc{\#1}}
\newcommand{\jl}{\commentaire{blue}} % Jeremy
\newcommand{\jlc}[1]{\remarque{blue}{(jl) #1}} %Jeremy

\newcommand{\myparagraph}[1]{{\noindent\textbf{#1}}}



==> sec/preli.tex <==
\section{Preliminary Study: Terrestrial Validation}
\label{sec:preliminary_study}

Before deploying MASt3R on lunar imagery, we investigate whether domain adaptation is necessary by conducting a controlled terrestrial validation study. 
Initial experiments revealed that MASt3R fails to reconstruct lunar topography when applied directly, producing predominantly flat point clouds. 
This failure could stem from two potential factors: (i) insufficient representation of aerial viewpoints in the training data, or (ii) the inherently low-texture characteristics of lunar surfaces.

To isolate these contributing factors, we designed a terrestrial experiment using aerial imagery of the French Pyrenees. 
This region provides an ideal testbed, combining diverse topographical features with varying texture densities while minimizing urban interference that could confound our analysis (\cref{fig:preliminary-pyrenees}). 
Our dataset comprises a high-resolution Digital Elevation Model (DEM) \sout{from the \textit{Institut national de l'information géographique et forestière} \textit{(IGN)}}   paired with corresponding orthophotography made publicly avialable by the \textit{IGN} \cite{ign_rgealti}. \gmc{Try to be more precise on the experimental setup: how many images on your dataset, and did you take a pretrained Master ? }
\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{ICCV2025-Author-Kit-Feb/images/preliminary_page-0001.jpg}
    \caption{Terrestrial validation region in the French Pyrenees, showcasing diverse topographical features and texture variations that mirror challenges expected in lunar reconstruction tasks. (\cg{Police moche})}
    \label{fig:preliminary-pyrenees}
\end{figure}

Our experimental results \sout{reveal nuanced performance characteristics that} \gmc{what I striked through is not very informative I think...} provide crucial insights for lunar domain transfer: 
as shown in \cref{tab:prelim-results-wide}, MASt3R achieves competitive pose estimation accuracy, with performance metrics comparable to those reported on the Co3Dv2 benchmark \gmc{these results are for which kind of scenes ?}. 
Specifically, the method achieves perfect rotation accuracy at \ang{5} tolerance and demonstrates robust performance across different angular thresholds. \gmc{I am not sure how this estimation measure works. Are these classical, or the ones for this dataset ? what does it mean \ang{5} or \ang{10} for a translation ?}

However, a critical finding emerges regarding texture dependency in 3D reconstruction quality. 
In regions with rich textural information, MASt3R maintains \gm{offers} a reliable geometric reconstruction. 
Conversely, in low-texture areas characteristic of snow cover and uniform grasslands, reconstruction fidelity degrades significantly, as evidenced by elevated RMSE and Chamfer distance metrics. \gmc{to convince the reader, you should put some evidence there, or say "we observed that"...}

\begin{table*}[t]
\centering
\caption{Quantitative performance analysis comparing terrestrial aerial reconstruction with MASt3R's Co3Dv2 benchmark results. 
Pose accuracy is measured using rotation (RRA) and translation (RTA) accuracy at \ang{5} and \ang{10} thresholds.}
\label{tab:prelim-results-wide}
\begin{tabular}{|c|cc|cc|ccc|}
\hline
\multirow{2}{*}{Dataset} & \multicolumn{2}{c|}{Pose @ \ang{5} (\%)} & \multicolumn{2}{c|}{Pose @ \ang{10} (\%)} & \multicolumn{3}{c|}{3D Reconstruction Metrics} \\
 & RRA & RTA & RRA & RTA & Reprojection
 (px) & RMSE (m) & Chamfer (m) \\
\hline
Terrestrial Pyrenees & 100.0 & 53.0 & 100.0 & 81.6 & 33.48 & 33.60 & 14.85 \\
MASt3R Co3Dv2 & 99.69 & 77.23 & 100.0 & 91.96 & -- & -- & -- \\
\hline
\end{tabular}
\end{table*}

These findings establish two key insights that directly inform our approach to lunar reconstruction. 
First, MASt3R demonstrates inherent capability for processing aerial viewpoints, confirming that viewpoint geometry alone does not explain the failure on lunar imagery. 
Second, the pronounced texture dependency observed in terrestrial low-texture regions strongly suggests that the sparse textural characteristics of lunar surfaces represent the primary challenge for \sout{direct application} \gm{adapting MASt3R to lunar elevation reconstruction.} .

This validation study thus provides compelling motivation for our domain-specific fine-tuning strategy, establishing that adaptation is necessary not due to viewpoint limitations but rather to address the unique textural challenges inherent in lunar surface reconstruction.
